Some graphical aspects of Frobenius structures

We survey some aspects of Frobenius algebras, Frobenius structures and their relation to finite Hopf algebras using graphical calculus. We focus on the `yanking' moves coming from a closed structure in a rigid monoidal category, the topological move, and the `yanking' coming from the Frobenius bilinear form and its inverse, used e.g. in quantum teleportation. We discus how to interpret the associated information flow. Some care is taken to cover non-symmetric Frobenius algebras and the Nakayama automorphism. We review graphically the Larson-Sweedler-Pareigis theorem showing how integrals of finite Hopf algebras allow to construct Frobenius structures. A few pointers to further literature are given, with a subjective tendency to graphically minded work.

==> bfmacros.tex <==
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{times}
\usepackage{hyperref}
\usepackage{graphicx}
\usepackage[arrow, matrix, curve, 2cell]{xy}
\usepackage{tikz}
%\usepackage{makeidx}  %% not needed (why?)
%\makeindex
%\usepackage{showlabels}

\let\today=\date
\setcounter{page}{1}     % set correct page number here
%% use this command to produce breakable formulae
%% may be used for particular formulae by {\allowdisplaybreaks <formula>}
%\allowdisplaybreaks
%% alternatively use \displaybreak[n] for n=0,1,2,3,4 (4 forces break)
%% no optional argument [n] implies n=4
%% \displaybreak[0]

%\setcounter{chapter}{1}  % set correct chapter number here
%\renewcommand{\baselinestretch}{1.0} %
%%
%% introduce a counter for the \mybenv \myeenv environment and set
%% it to be reset for each section, as done for equations
%%
\newcounter{mycnt}
\def\themycnt{\thesection.\arabic{mycnt}}
\def\mybenv#1{\refstepcounter{mycnt}%
       \vskip 3pt\noindent{\bf #1~~\themycnt}:~}
\def\myeenv{\hfill\rule{1ex}{1ex}\vskip 3pt}
\def\qed{\hfill$\Box$}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%%  add the counter equation to the reset list, reset section wise
%%  (needs @ to be made an ordinary letter, and undo that thereafter
%%
\makeatletter
\@addtoreset{equation}{section}
\@addtoreset{mycnt}{section}
\makeatother
%
%
\renewcommand{\theequation}{\arabic{section}-\arabic{equation}}
%
\mathsurround 1.5pt
%
%%%
%%% Macros needed
%%%
\def\nn{\nonumber \\}
\def\Id{\text{I\!d}}
\def\calE{\mathcal{E}}
\def\calH{\mathcal{H}}
\def\calM{\mathcal{M}}
\def\sfm{\textsf{m}}
\def\sfS{\textsf{S}}
\def\sfH{\mathsf{H}}
\def\sfR{\mathsf{R}}
\def\sfT{\mathsf{T}}
\def\antip{{\textsf S}}
\def\Bil{\mathsf{Bil}^r_{ass}}
\def\eval{\textsf{ev}}
\def\ceval{\textsf{cev}}
\def\la{\langle}
\def\ra{\rangle}
\def\LR{\mathbf{l}}
\def\RR{\mathbf{r}}
\def\!{\kern -0.15ex}
\def\barbeta{\overline{\beta}}
\def\baralpha{\overline{\alpha}}
\def\Hom{\mathrm{Hom}}
\def\End{\mathrm{End}}
\def\Aut{\mathrm{Aut}}
\def\Der{\mathrm{Der}}
\def\InnDer{\mathrm{InnDer}}
\def\Ext{\mathrm{Ext}}
\def\Ker{\mathrm{Ker}}
\def\Pic{\mathrm{Pic}}

